Parameterized Complexity of Segment Routing

Segment Routing is a recent network technology that helps optimizing network throughput by providing finer control over the routing paths. Instead of routing directly from a source to a target, packets are routed via intermediate waypoints. Between consecutive waypoints, the packets are routed according to traditional shortest path routing protocols. Bottlenecks in the network can be avoided by such rerouting, preventing overloading parts of the network. The associated NP-hard computational problem is Segment Routing: Given a network on $n$ vertices, $d$ traffic demands (vertex pairs), and a (small) number $k$, the task is to find for each demand pair at most $k$ waypoints such that with shortest path routing along these waypoints, all demands are fulfilled without exceeding the capacities of the network. We investigate if special structures of real-world communication networks could be exploited algorithmically. Our results comprise NP-hardness on graphs with constant treewidth even if only one waypoint per demand is allowed. We further exclude (under standard complexity assumptions) algorithms with running time $f(d) n^{g(k)}$ for any functions $f$ and $g$. We complement these lower bounds with polynomial-time solvable special cases.

==> figures/treewidth.tex <==
\usetikzlibrary{shadows.blur,arrows.meta}
\usetikzlibrary{chains,positioning,backgrounds,mindmap,intersections,shapes}
\usetikzlibrary{calc}
\begin{tikzpicture}
%\tikzstyle{mvertex}=[thick,circle,inner sep=0.05cm, minimum size=3mm,draw, fill=gray!50!white,blur shadow={shadow xshift=0.25ex, shadow yshift=-0.25ex, shadow opacity=60, shadow blur radius=0.2ex}]
\tikzstyle{mvertex}=[small black vertex]
\tikzstyle{medge}=[black edge]

  \node (t1) {
      \begin{tikzpicture}[level distance=0.75cm,medge,
              level 1/.style={sibling distance=0.75cm},
              level 2/.style={sibling distance=0.75cm}]
          \node[mvertex,fill=black,minimum size=2mm] (A) {}
          child {node[mvertex,fill=black,minimum size=2mm] (B) {}
                  child {node[mvertex,fill=black,minimum size=2mm] (D) {}}
                  child {node[mvertex,fill=black,minimum size=2mm] (E) {}}}
          child {node[mvertex,fill=black,minimum size=2mm] (C) {}};
      \end{tikzpicture}
  };

  \node[text width=1.5cm, below = of t1, yshift=1cm] {tw = $1$};

  \node[right = of t1] (t2) {
      \begin{tikzpicture}
          \coordinate (A) at (90:1);
          \coordinate (B) at (162:1);
          \coordinate (C) at (234:1);
          \coordinate (D) at (306:1);
          \coordinate (E) at (18:1);

          \draw[medge] (A) -- (B) -- (C) -- (D) -- (E) -- (A);

          \foreach \vertex in {A,B,C,D,E}
          \filldraw (\vertex) circle (3pt);
      \end{tikzpicture}
  };

  \node[text width=1.5cm, below = of t2, yshift=1cm] {tw = $2$};

  \node[right = of t2] (t3) {
      \begin{tikzpicture}
          \foreach \x in {0,1,2} {
                  \foreach \y in {0,1,2} {
                          \node[mvertex,fill=black,minimum size=2mm] (\x\y) at (\x,\y) {};
                      }
              }

          \foreach \x in {0,1,2} {
                  \foreach \y in {0,1,2} {
                          \foreach \xx in {0,1,2} {
                                  \foreach \yy in {0,1,2} {
                                          \ifnum \x<\xx
                                              \ifnum \y=\yy
                                                  \draw[medge] (\x\y) -- (\xx\yy);
                                              \fi
                                          \fi
                                          \ifnum \x=\xx
                                              \ifnum \y<\yy
                                                  \draw[medge] (\x\y) -- (\xx\yy);
                                              \fi
                                          \fi;
                                      }
                              }
                      }
              }
      \end{tikzpicture}
  };

  \node[text width=1.5cm, below = of t3, yshift=1cm] {tw = $\sqrt{n}$};

  \node[right = of t3] (t4) {
      \begin{tikzpicture}
          \foreach \a in { 18, 90, 162, 234, 306 } {
                  \foreach \b in { 18, 90, 162, 234, 306 } {
                          \draw[medge] (\a:1) -- (\b:1);
                      }
              }

          \foreach \a in {18,90, 162, 234, 306 } {
                  \filldraw (\a:1) circle (3pt);
              }
      \end{tikzpicture}
  };

  \node[text width=1.5cm, below = of t4, yshift=1cm] {tw = $n$};
\end{tikzpicture}
